Final results on the $0\nu\beta\beta$ decay half-life limit of $^{100}$Mo from the CUPID-Mo experiment

The CUPID-Mo experiment to search for 0$\nu\beta\beta$ decay in $^{100}$Mo has been recently completed after about 1.5 years of operation at Laboratoire Souterrain de Modane (France). It served as a demonstrator for CUPID, a next generation 0$\nu\beta\beta$ decay experiment. CUPID-Mo was comprised of 20 enriched Li$_2$$^{100}$MoO$_4$ scintillating calorimeters, each with a mass of $\sim$ 0.2 kg, operated at $\sim$20 mK. We present here the final analysis with the full exposure of CUPID-Mo ($^{100}$Mo exposure of 1.47 kg$\times$yr) used to search for lepton number violation via 0$\nu\beta\beta$ decay. We report on various analysis improvements since the previous result on a subset of data, reprocessing all data with these new techniques. We observe zero events in the region of interest and set a new limit on the $^{100}$Mo 0$\nu\beta\beta$ decay half-life of $T^{0\nu}_{1/2} > 1.8 \times 10^{24}$ year (stat.+syst.) at 90% CI. Under the light Majorana neutrino exchange mechanism this corresponds to an effective Majorana neutrino mass of $\left<m_{\beta \beta}\right> < (0.28$--$0.49)$ eV, dependent upon the nuclear matrix element utilized.

==> 05psd_old.tex <==
\section{Pulse-Shape Discrimination}
\label{sec:psd}
There are some pulses in the data stream that are abnormal compared to the typical pulse shape. These pathological pulses arise due to various issues, such as energy deposit to the NTD itself, baseline jumps during the pulse, large few sample spikes or deficiencies in the digitization, and pileup. All these effects cause the OF amplitude reconstruction to be biased and can result in incorrect energy values being assigned to these events. Such effects, mainly due to pileup, are expected to be a leading contributor to the background at high energies near \qbb. These events can be removed via pulse-shape discrimination (PSD) cuts which define some set of metrics with which to characterize the typical shape of a pulse.

In \Q a pulse-shape discriminator, referred to as ``pulse-shape analysis" (PSA) was developed and used for earlier analyses~\cite{CUOREPRL2017}. PSA examines several pulse-shape parameters: baseline slope, a goodness of fit on the  left / right side of  the pulse (test-value-left / test-value-right, or TVL and TVR, respectively), OF time delay, and the OF pulse decay and rise times. This is done on $\gamma$ events in the energy range of 500-2600~\,keV and a set of empirical fits to the median and median absolute deviation (MAD) of the parameter values as a function of energy are constructed, on a channel-dataset basis. These parameters are then normalized and a multidimensional Mahalanobis distance is computed to set a cut threshold. The TVL/TVR quantities are $\chi^2$ like quantities that describe the goodness of fit between an optimum filtered pulse and the filtered average pulse template used in the construction of the OF. Of relevance for this analysis will be the normalized TVL and TVR quantities (NormTVL and NormTVR) which are used to provide an additional rejection of types of pileup~\cite{PhysRevC.104.015501}.

In the earlier CUPID-Mo analysis~\cite{CuMoPRL} and recent \Q 1-ton-yr \cite{CUORE1ton} a new method utilizing principle component analysis (PCA) was implemented~\cite{PCA_Huang_2021}. This method uses 2\vbb events to derive a set of principle components that describe typical pulse shapes for each channel-dataset. As one utilizes more components the combination better represents the ensemble of training pulses utilized. Typically, the leading component is similar to the average pulse with subsequent components adding information about pulse time offsets and derivative and characteristic noise. Ultimately these are used to construct a term referred to as the reconstruction error (R) which describes how well a single pulse, $\bf{x}$, matches the $m$ principle components utilized:
\begin{equation}
    R = \sqrt{\sum_{i=1}^{n}{\left(x_{i} - \sum_{a=1}^{m}{q_{a}w_{a,i}}\right)^{2}}},
\end{equation}
where $\mathbf{w_{a}}$ is the $a$-th eigenvector of the PCA with the projection of $\mathbf{x}$ onto each component given by $q_{a} = \mathbf{x}\cdot\mathbf{w}_{a}$. The RE is then normalized to remove the energy dependence of the distribution, creating the normalized reconstruction error (NRE) upon which a flat cut is defined.


\subsection{PCA Improvements}
\label{sec:pca}
In this work several aspects of the PCA cut used previously were improved upon. In particular, the training sample was further cleaned, the normalization process was adjusted to occur on a run-by-run basis and to have the energy dependence of the MAD accounted for, and the rejection power was improved. The utilization of more than a single PCA component is one possible way to improve the rejection power of the cut while maintaining a high efficiency. Higher order components are more susceptible to distortion in the presence of abnormal pulses leaking into the training sample. This is mitigated by the use of a stricter training cut that requires the pre-trigger baseline RMS not be identically zero (indicative of saturation and subsequent baseline jumps), and a simple pulse counting algorithm must identify no more than a single pulse on the LMO and a single pulse in the LD in the event window. This selection criterion resulted in a mild reduction in the size of the training sample but greatly improves the purity against abnormal pulse shapes, allowing higher order principle components to be utilized.


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/ch1_ds8248_pcaFail1.pdf}
    \includegraphics[width=0.5\textwidth]{Figures/ch1_ds8248_pcaPileup.pdf}
    \caption{Two examples of events that are rejected due to the PSD cut. The event in the top is an example of possible pileup with another faster event class along with a noise glitch. Both of these features alone would be sufficient to cause the optimum filter to fail to reconstruct the proper event energy due to possible ringing effects in the filter due to faster than expected features. The event in the bottom is an example of a pileup event as well but more separated in time. In this case the proximity is still such that it may result in the optimum filter improperly estimating the amplitude, and the left-most pulse would bias the mean of the pre-pulse baseline that is used for amplitude estimation.}
        \label{fig:pcaFail}

\end{figure}

The normalization of the RE was improved by changing the algorithm to utilize individual runs to characterize the typical RE in a given energy range as opposed to the entire dataset. This allows for runs that are more noisy to not be biased when compared against the whole dataset and allows calibration runs to also be self-normalized. While statistics are robust enough for correction of the typical RE value as a function of energy, the correction of the MAD as a function of energy requires the whole aggregate set of statistics. Here we characterize the energy dependence of the MAD for all channels in a dataset together to get a linear fit to the global energy dependence. This global energy dependent function is then rescaled by ratio of the individual channel flat MAD and flat global MAD to give an approximate channel-based rescaling.  Taken together these two adjustments result in a tighter core distribution of the NRE.
\begin{figure}[htpb]
    \label{fig:nre}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/pca_nve_color.pdf}
    \caption{The normalized reconstruction error as a function of energy for a single channel-dataset. One can see that relative to the unnromalized version the energy dependence has been corrected for allowing for the possiblity of an energy-independent cut threshold to be set.}
\end{figure}

Finally, by examining the overall efficiency as a function of number of PCA components and the impact on the 2615~\,keV peak resolution, and examination from optimizing the sensitivity via Cowan's metric, we set an improved PCA cut defined on 6 components.

\subsection{PSD Enhancements}
\label{sec:psd_enhance}
The six-component based PCA cut has a relatively high efficiency and rejects obvious abnormal pulses (see Fig.~\ref{fig:pcaFail}). However it is observed that some pile-up type events still leak through this cut alone. It is observed that the PSA based TVL and TVR cuts are able to remove a large portion of these with negligible loss to efficiency. The discrimination power from these two cuts is a result of these quantities being defined from the OF pulse shape which has a better signal-to-noise ratio and hence an easier time discerning instances of small-scale pileup events that the PCA method misses.  We combine the various pulse-shape cuts to form the ultimate PSD cut by requiring that $|\mathrm{NRE}|<9$ and that the absolute values of both NormTVL and NormTVR both be $<10$.

The resulting cut maintains a high efficiency, comparable to the previous analysis (see Sect.~\ref{sec:eff}) while rejecting abnormal events more robustly.


==> 06apsdbad.tex <==
\section{Pulse-Shape Discrimination}
\label{sec:psd}
A significant contribution to the background near \qbb are pile-up events in which two or more events overlap to various degrees. This can cause incorrect amplitude estimation and shift events into, or out of, our region of interest. In order to mitigate this effect we employ a pulse shape discrimination cut that is comprised of two different techniques.

The main method we utilize for PSD is a cut based on principle component analysis (PCA) as was originally utilized in the previous analysis~\cite{CuMoPRL, PCA_Huang_2021}, and successfully applied recently to \Q~\cite{CUORE1ton}. This method utilizes 2\vbb events between $1-2$~\,MeV to derive a set of principle components that can be used to describe typical pulse shapes for each channel-dataset. The leading principle component typically resembles the average pulse template with subsequent components adding small adjustments. These are used to compute a reconstruction error ($R$) for every event that characterizes how well a given pulse, $\bf{x}$, matches the set of principle components, $m$, utilized:
\begin{equation}
    R = \sqrt{\sum_{i=1}^{n}{\left(x_{i} - \sum_{a=1}^{m}{q_{a}w_{a,i}}\right)^{2}}},
\end{equation}
where $\mathbf{w_{a}}$ is the $a$-th eigenvector of the PCA with the projection of $\mathbf{x}$ onto each component given by $q_{a} = \mathbf{x}\cdot\mathbf{w}_{a}$. Typically $R$ posesses some energy dependence that is then normalized by subtracting away the linear component and scaling by the median absolute deviation (MAD). The resulting normalized reconstruction error, $N$ is then used with a flat threshold to reject abnormal events.

\subsection{PCA Improvements}
\label{sec:pca}
In this work several aspects of the PCA cut used previously are improved upon. In particular, the training sample is further cleaned, the normalization process now occurs on a run-by-run basis and the energy dependence of the MAD is also incorporated in the normalization. As higher order components are more susceptible to distortion in the presence of abnormal pulses in the training sample, a stricter selection cut is used: we require that the pretrigger baseline RMS not be identically zero (indicative of digitizer saturation and subsequent baseline jumps), and that a simple pulse counting algorithm must identify no more than 1 pulse on the LMO and primary LD in the event window. This selection criterion results in a mild reduction in the size of the training sample but greatly improves the training sample purity allowing higher order principle components to be utilized which improves the rejection power of this cut while maintaining relatively high efficiency.

\begin{figure*}[ht!]
    \centering
    \begin{minipage}{0.6\textwidth}
        \includegraphics[width=\linewidth]{Figures/pca_vs_energy_ch1.pdf}
    \end{minipage}
    \begin{minipage}{0.38\textwidth}
        \includegraphics[width=\linewidth]{Figures/pca_ch1_pileup.pdf}
        \includegraphics[width=\linewidth]{Figures/pca_ch1_ok.pdf}
    \end{minipage}
    \caption{Example of the normalized PCA reconstruction error (\textit{left}) as a function of energy, and two types of events (\textit{right}) that exist in our data. (\textit{left:}) The normalized reconstruction errors have no energy dependence and are normalized on a run-by-run basis for each channel allowing for a single flat cut to be applied across all channels in every dataset. Events with higher normalized reconstruction errors are removed due to likely having incorrect energy values which may cause such events to be shifted into, or out of, the region of interest. (\textit{right}): The top event is an example of a pile-up event with high normalized reconstruction error ($\sim$22) which would have an incorrect amplitude reconstruction. The bottom event is a more typical pulse with a small normalized reconstruction error ($\sim$0.5), having no resulting error in its OF amplitude reconstruction.
    }
     \label{fig:pcaFail}
\end{figure*}

The normalization of the reconstruction error is performed on a run-by-run basis as opposed to whole-dataset. This change allows for an improved normalization that better reflects run-to-run changes in $R$ that may arise due to variations in noise. While statistics are robust for normalization of the reconstruction error, the energy dependence of the MAD requires aggregate statistics of the whole dataset. We characterize the energy dependence for all channels in a dataset with a linear model and flat fit (as was done originally for the individual channel fits) and then scale the individual channel MAD values by ratio of the ensemble linear and flat fits to provide a proxy for channel based energy scaling.

Finally, by examining the overall efficiency as a function of number of PCA components, the impact on the 2615~\,keV peak resolution, and examination from optimizing the median discovery significance as suggested in Cowan et al.~\cite{CowanMetric}, we set an improved PCA cut defined on 6 components.

\subsection{PSD Enhancements}
\label{sec:psd_enhance}
To finalize the PSD cut we utilize a two additional parameters developed in previous \Q analyses~\cite{CUOREPRL2017}. These parameters are computed on the optimally filtered pulse itself and are measures of goodness of fit on the left/right side of the filtered pulse, referred to as test-value-left, test-value-right, or TVL and TVR respectively. These $\chi^2$-like quantities are normalized via empirical fits of their median and MAD energy dependencies using $\gamma$ events from 500-2600~\,keV. As these quantities are computed on the filtered pulses they provide an additional proxy to detect subtle pulse-shape deviations and provide a complimentary way to reject pile-up events~\cite{PhysRevC.104.015501}.

The six-component based PCA cut has a relatively high efficiency and rejects obvious abnormal pulses (see Fig.~\ref{fig:pcaFail}). However we observe that some pile-up type events still leak through this cut alone. The TVL and TVR cuts are able to remove a large portion of these with negligible loss to efficiency. The discrimination power from these two cuts arises from the fact they are derived on the optimally filtered waveforms. They are sensitive to pile-up in a fashion that the PCA is not and owing to the better signal-to-noise ratio, tend reject small-scale pileup events that the PCA cut is insensitive to. We combine the various pulse-shape cuts to form the final PSD cut by requiring that the absolute value of the normalized reconstruction error be less than nine, and that both the absolute value of the normalized TVR and TVL quantities be less than ten. The resulting cut maintains an efficiency comparable to the previous analysis (see Sect.~\ref{sec:eff}) while being able to reject more types of abnormal events.


==> 99spares.tex <==
\subsection{Trigger Thresholds}
The trigger threshold for the OT utilized is evaluated by injection of ideal pulses into noise events with different scaling and then running this data through the same OT used in triggering the data. This is accomplished by selecting a wide range of possible energy values, and running the energy calibration steps backwards: from a known energy one can extract the stabilized OF amplitude and then from this the raw pulse amplitude with which to scale the idealized pulse. This is done on noise events throughout an entire dataset for each channel. The pseudo-raw pulse is then run through the OT used for that channel-dataset and we examine if the OT issues a trigger or not. From this we build up a sample of the trigger efficiency as a function of injected energy which is then fit to an error function to determine the energy at which 90\% of injected triggers are found. We find that the median 90\% trigger efficiency for LMO channels is 8.5~\,keV and for LD's 0.55~\,keV. This is well below the analysis threshold of 40~\,keV used for this analysis. We remark also that the OT threshold itself was set at a very conservative level equivalent to ten times the average noise width as defined by the ANPS. It is probable that the threshold could be lowered more with some investigation, with possible applications in searches requiring lower energy thresholds, such as low-mass inelastic dark matter searches.

\begin{figure}[htpb]
    \label{fig:ot_thresh}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/thrshold_distri_lmo.pdf}
    \includegraphics[width=0.5\textwidth]{Figures/thrshold_distri.pdf}
    \caption{\emph{Top:} Distribution of trigger thresholds for all channel-dataset pairs in this analysis. The red dashed line represents the analysis threshold of 40~\,keV set in the anti-coincidence selection. The vast majority of trigger thresholds below 20~\,keV with median threshold of 8.5~\,keV. \emph{Bottom:}Distribution of trigger thresholds for light detectors. The LD's have a much lower trigger threshold compared to the LMO's and have a median 90\% trigger threshold of 0.55~\,keV.
    \brad{Need to remake these to remove titles and statbox. Also check if Ch3 is included.}
    \toby{switch to log x}
    }
\end{figure}

==> authorlist.tex <==
\author{
E.~Armengaud\thanksref{CEA-IRFU}\and
C.~Augier\thanksref{IPNL}\and
A.~S.~Barabash\thanksref{ITEP}\and
F.~Bellini\thanksref{Sapienza,INFN-Roma}\and
G.~Benato\thanksref{LNGS}\and
A.~Beno\^{\i}t\thanksref{Neel}\and
M.~Beretta\thanksref{UCB}\and
L.~Berg\'e\thanksref{IJCLab}\and
J.~Billard\thanksref{IPNL}\and
Yu.~A.~Borovlev\thanksref{NIIC}\and
Ch.~Bourgeois\thanksref{IJCLab}\and
V.~B.~Brudanin\thanksref{JINR}\and
P.~Camus\thanksref{Neel}\and
L.~Cardani\thanksref{INFN-Roma}\and
N.~Casali\thanksref{INFN-Roma}\and
A.~Cazes\thanksref{IPNL}\and
M.~Chapellier\thanksref{IJCLab}\and
F.~Charlieux\thanksref{IPNL}\and
D.Chiesa\thanksref{Milano,INFN-Milano}\and
M.~de~Combarieu\thanksref{CEA-IRAMIS}\and
I.~Dafinei\thanksref{INFN-Roma}\and
F.~A.~Danevich\thanksref{KINR}\and
M.~De~Jesus\thanksref{IPNL}\and
T.~Dixon\thanksref{UCB}\and
L.~Dumoulin\thanksref{IJCLab}\and
K.~Eitel\thanksref{KIT-IK}\and
F.~Ferri\thanksref{CEA-IRFU}\and
B.~K.~Fujikawa\thanksref{LBNLNSD}\and
J.~Gascon\thanksref{IPNL}\and
L.~Gironi\thanksref{Milano,INFN-Milano}\and
A.~Giuliani\thanksref{e1,IJCLab}\and
V.~D.~Grigorieva\thanksref{NIIC}\and
M.~Gros\thanksref{CEA-IRFU}\and
E.~Guerard\thanksref{IJCLab}\and
D.~L.~Helis\thanksref{CEA-IRFU}\and
H.~Z.~Huang\thanksref{Fudan}\and
R.~Huang\thanksref{UCB}\and
J.~Johnston\thanksref{MIT}\and
A.~Juillard\thanksref{IPNL}\and
H.~Khalife\thanksref{IJCLab}\and 
M.~Kleifges\thanksref{KIT-IPE}\and
V.~V.~Kobychev\thanksref{KINR}\and
Yu.~G.~Kolomensky\thanksref{UCB,LBNLPH}\and
S.I.~Konovalov\thanksref{ITEP}\and
A.~Leder\thanksref{MIT}\and
P.~Loaiza\thanksref{IJCLab}\and
L.~Ma\thanksref{Fudan}\and
E.~P.~Makarov\thanksref{NIIC}\and
P.~de~Marcillac\thanksref{IJCLab}\and
R.~Mariam\thanksref{IJCLab}\and
L.~Marini\thanksref{UCB, LBNLNSD, LNGS}\and
S.~Marnieros\thanksref{IJCLab}\and
D.~Misiak\thanksref{IPNL}\and
X.-F.~Navick\thanksref{CEA-IRFU}\and
C.~Nones\thanksref{CEA-IRFU}\and
E.B.~Norman\thanksref{UCB}\and
V.~Novati\thanksref{IJCLab}\and
E.~Olivieri\thanksref{IJCLab}\and
J.~L.~Ouellet\thanksref{MIT}\and
L.~Pagnanini\thanksref{Milano,INFN-Milano}\and
P.~Pari\thanksref{CEA-IRAMIS}\and
L.~Pattavina\thanksref{LNGS,TUM}\and
B.~Paul\thanksref{CEA-IRFU}\and
M.~Pavan\thanksref{Milano,INFN-Milano}\and
H.~Peng\thanksref{USTC}\and
G.~Pessina\thanksref{INFN-Milano}\and
S.~Pirro\thanksref{LNGS}\and
D.~V.~Poda\thanksref{IJCLab}\and
O.~G.~Polischuk\thanksref{KINR}\and
S.~Pozzi\thanksref{INFN-Milano}\and
E.~Previtali\thanksref{Milano,INFN-Milano}\and
Th.~Redon\thanksref{IJCLab}\and
A.~Rojas\thanksref{LSM}\and
S.~Rozov\thanksref{JINR}\and 
C.~Rusconi\thanksref{USC}\and
V.~Sanglard\thanksref{IPNL}\and
J.A.~Scarpaci\thanksref{IJCLab}\and
K.~Sch\"affner\thanksref{LNGS}\and
B.~Schmidt\thanksref{LBNLNSD}\and
Y.~Shen\thanksref{Fudan}\and
V.~N.~Shlegel\thanksref{NIIC}\and
B.~Siebenborn\thanksref{KIT-IK}\and
V.~Singh\thanksref{UCB}\and
C.~Tomei\thanksref{INFN-Roma}\and
V.~I.~Tretyak\thanksref{KINR}\and 
V.~I.~Umatov\thanksref{ITEP}\and
L.~Vagneron\thanksref{IPNL}\and
M.~Vel\'azquez\thanksref{UGA}\and
B.~Welliver\thanksref{UCB}\and
L.~Winslow\thanksref{MIT}\and
M.~Xue\thanksref{USTC}\and
E.~Yakushev\thanksref{JINR}\and
M.~Zarytskyy\thanksref{KINR}\and
A.~S.~Zolotarova\thanksref{IJCLab}
}

\thankstext{e1}{e-mail: andrea.giuliani@ijclab.in2p3.fr}

\institute{
IRFU, CEA, Universit\'{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France  \label{CEA-IRFU} \and 
Univ Lyon, Universit\'{e} Lyon 1, CNRS/IN2P3, IP2I-Lyon, F-69622, Villeurbanne, France  \label{IPNL} \and 
National Research Centre Kurchatov Institute, Institute of Theoretical and Experimental Physics, 117218 Moscow, Russia  \label{ITEP} \and 
Dipartimento di Fisica, Sapienza Universit\`a di Roma, P.le Aldo Moro 2, I-00185, Rome, Italy \label{Sapienza} \and 
INFN, Sezione di Roma, P.le Aldo Moro 2, I-00185, Rome, Italy \label{INFN-Roma} \and
Department of Physics, University of California, Berkeley, California 94720, USA \label{UCB} \and
CNRS-N\'eel, 38042 Grenoble Cedex 9, France \label{Neel} \and
Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, I-20126 Milano, Italy \label{Milano} \and 
INFN, Sezione di Milano-Bicocca, I-20126 Milano, Italy \label{INFN-Milano} \and 
Nikolaev Institute of Inorganic Chemistry, 630090 Novosibirsk, Russia \label{NIIC} \and
Université Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France \label{IJCLab} \and
Laboratory of Nuclear Problems, JINR, 141980 Dubna, Moscow region, Russia \label{JINR} \and
IRAMIS, CEA, Universit\'{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France \label{CEA-IRAMIS} \and
Institute for Nuclear Research, 03028 Kyiv, Ukraine \label{KINR} \and 
Karlsruhe Institute of Technology, Institut f\"{u}r Kernphysik, 76021 Karlsruhe, Germany \label{KIT-IK} \and
Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA \label{LBNLNSD} \and
Key Laboratory of Nuclear Physics and Ion-beam Application (MOE), Fudan University, Shanghai 200433, PR China \label{Fudan} \and
Massachusetts Institute of Technology, Cambridge, MA 02139, USA \label{MIT} \and
Karlsruhe Institute of Technology, Institut f\"{u}r Prozessdatenverarbeitung und Elektronik, 76021 Karlsruhe, Germany \label{KIT-IPE} \and 
Physics Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA \label{LBNLPH} \and
INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi (AQ), Italy \label{LNGS} \and
LSM, Laboratoire Souterrain de Modane, 73500 Modane, France \label{LSM} \and
Physik Department, Technische Universit\"at M\"unchen, Garching D-85748, Germany \label{TUM} \and
Department of Modern Physics, University of Science and Technology of China, Hefei 230027, PR China \label{USTC} \and
Department of Physics and Astronomy, University of South Carolina, SC 29208, Columbia, USA \label{USC} \and
Universit\'e Grenoble Alpes, CNRS, Grenoble INP, SIMAP, 38402 Saint Martin d'H\'eres, France \label{UGA} 
}
 


==> authorlist_old.tex <==
\author{
E.~Armengaud\thanksref{CEA-IRFU}\and
C.~Augier\thanksref{IPNL}\and
A.~S.~Barabash\thanksref{ITEP}\and
F.~Bellini\thanksref{Sapienza,INFN-Roma}\and
G.~Benato\thanksref{UCB}\and
A.~Beno\^{\i}t\thanksref{Neel}\and
M.~Beretta\thanksref{Milano,INFN-Milano}\and
L.~Berg\'e\thanksref{CSNSM}\and
J.~Billard\thanksref{IPNL}\and
Yu.~A.~Borovlev\thanksref{NIIC}\and
Ch.~Bourgeois\thanksref{LAL}\and
M.~Briere\thanksref{LAL}\and
V.~B.~Brudanin\thanksref{JINR}\and
P.~Camus\thanksref{Neel}\and
L.~Cardani\thanksref{INFN-Roma}\and
N.~Casali\thanksref{INFN-Roma}\and
A.~Cazes\thanksref{IPNL}\and
M.~Chapellier\thanksref{CSNSM}\and
F.~Charlieux\thanksref{IPNL}\and
M.~de~Combarieu\thanksref{CEA-IRAMIS}\and
I.~Dafinei\thanksref{INFN-Roma}\and
F.~A.~Danevich\thanksref{KINR}\and
M.~De~Jesus\thanksref{IPNL}\and
L.~Dumoulin\thanksref{CSNSM}\and
K.~Eitel\thanksref{KIT-IK}\and
E.~Elkhoury\thanksref{IPNL}\and
F.~Ferri\thanksref{CEA-IRFU}\and
B.~K.~Fujikawa\thanksref{LBNLNSD}\and
J.~Gascon\thanksref{IPNL}\and
L.~Gironi\thanksref{Milano,INFN-Milano}\and
A.~Giuliani\thanksref{e1,CSNSM,DISAT}\and
V.~D.~Grigorieva\thanksref{NIIC}\and
M.~Gros\thanksref{CEA-IRFU}\and
E.~Guerard\thanksref{LAL}\and
D.~L.~Helis\thanksref{CEA-IRFU}\and
H.~Z.~Huang\thanksref{Fudan}\and
R.~Huang\thanksref{UCB}\and
J.~Johnston\thanksref{MIT}\and
A.~Juillard\thanksref{IPNL}\and
H.~Khalife\thanksref{CSNSM}\and 
M.~Kleifges\thanksref{KIT-IPE}\and
V.~V.~Kobychev\thanksref{KINR}\and
Yu.~G.~Kolomensky\thanksref{UCB,LBNLPH}\and
S.I.~Konovalov\thanksref{ITEP}\and
A.~Leder\thanksref{MIT}\and
P.~Loaiza\thanksref{LAL}\and
L.~Ma\thanksref{Fudan}\and
E.~P.~Makarov\thanksref{NIIC}\and
P.~de~Marcillac\thanksref{CSNSM}\and
L.~Marini\thanksref{UCB, LBNLNSD, LNGS}\and
S.~Marnieros\thanksref{CSNSM}\and
D.~Misiak\thanksref{IPNL}\and
X.-F.~Navick\thanksref{CEA-IRFU}\and
C.~Nones\thanksref{CEA-IRFU}\and
V.~Novati\thanksref{CSNSM}\and
E.~Olivieri\thanksref{CSNSM}\and
J.~L.~Ouellet\thanksref{MIT}\and
L.~Pagnanini\thanksref{Milano,INFN-Milano}\and
P.~Pari\thanksref{CEA-IRAMIS}\and
L.~Pattavina\thanksref{LNGS,TUM}\and
B.~Paul\thanksref{CEA-IRFU}\and
M.~Pavan\thanksref{Milano,INFN-Milano}\and
H.~Peng\thanksref{USTC}\and
G.~Pessina\thanksref{INFN-Milano}\and
S.~Pirro\thanksref{LNGS}\and
D.~V.~Poda\thanksref{CSNSM,KINR}\and
O.~G.~Polischuk\thanksref{KINR}\and
E.~Previtali\thanksref{Milano,INFN-Milano}\and
Th.~Redon\thanksref{CSNSM}\and
S.~Rozov\thanksref{JINR}\and 
C.~Rusconi\thanksref{USC}\and
V.~Sanglard\thanksref{IPNL}\and
K.~Sch\"affner\thanksref{LNGS}\and
B.~Schmidt\thanksref{LBNLNSD}\and
Y.~Shen\thanksref{Fudan}\and
V.~N.~Shlegel\thanksref{NIIC}\and
B.~Siebenborn\thanksref{KIT-IK}\and
V.~Singh\thanksref{UCB}\and
S.~Sorbino\thanksref{Sapienza,INFN-Roma}\and
C.~Tomei\thanksref{INFN-Roma}\and
V.~I.~Tretyak\thanksref{KINR}\and 
V.~I.~Umatov\thanksref{ITEP}\and
L.~Vagneron\thanksref{IPNL}\and
M.~Vel\'azquez\thanksref{UGA}\and
M.~Weber\thanksref{KIT-IPE}\and
B.~Welliver\thanksref{LBNLNSD}\and
L.~Winslow\thanksref{MIT}\and
M.~Xue\thanksref{USTC}\and
E.~Yakushev\thanksref{JINR}\and
A.~S.~Zolotarova\thanksref{CSNSM}
}

\thankstext{e1}{e-mail: andrea.giuliani@csnsm.in2p3.fr}

\institute{
IRFU, CEA, Universit\'{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France  \label{CEA-IRFU} \and 
Univ Lyon, Universit\'{e} Lyon 1, CNRS/IN2P3, IP2I-Lyon, F-69622, Villeurbanne, France  \label{IPNL} \and 
National Research Centre Kurchatov Institute, Institute of Theoretical and Experimental Physics, 117218 Moscow, Russia  \label{ITEP} \and 
Dipartimento di Fisica, Sapienza Universit\`a di Roma, P.le Aldo Moro 2, I-00185, Rome, Italy \label{Sapienza} \and 
INFN, Sezione di Roma, P.le Aldo Moro 2, I-00185, Rome, Italy \label{INFN-Roma} \and
Department of Physics, University of California, Berkeley, California 94720, USA \label{UCB} \and
CNRS-N\'eel, 38042 Grenoble Cedex 9, France \label{Neel} \and
Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, I-20126 Milano, Italy \label{Milano} \and 
INFN, Sezione di Milano-Bicocca, I-20126 Milano, Italy \label{INFN-Milano} \and 
CSNSM, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, 91405 Orsay, France \label{CSNSM} \and
Nikolaev Institute of Inorganic Chemistry, 630090 Novosibirsk, Russia \label{NIIC} \and
LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, 91898 Orsay, France \label{LAL} \and
Laboratory of Nuclear Problems, JINR, 141980 Dubna, Moscow region, Russia \label{JINR} \and
IRAMIS, CEA, Universit\'{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France \label{CEA-IRAMIS} \and
Institute for Nuclear Research, 03028 Kyiv, Ukraine \label{KINR} \and 
Karlsruhe Institute of Technology, Institut f\"{u}r Kernphysik, 76021 Karlsruhe, Germany \label{KIT-IK} \and
Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA \label{LBNLNSD} \and
DISAT, Universit\`a dell'Insubria, 22100 Como, Italy \label{DISAT} \and
Key Laboratory of Nuclear Physics and Ion-beam Application (MOE), Fudan University, Shanghai 200433, PR China \label{Fudan} \and
Massachusetts Institute of Technology, Cambridge, MA 02139, USA \label{MIT} \and
Karlsruhe Institute of Technology, Institut f\"{u}r Prozessdatenverarbeitung und Elektronik, 76021 Karlsruhe, Germany \label{KIT-IPE} \and 
Physics Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA \label{LBNLPH} \and
INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi (AQ), Italy \label{LNGS} \and
Physik Department, Technische Universit\"at M\"unchen, Garching D-85748, Germany \label{TUM} \and
Department of Modern Physics, University of Science and Technology of China, Hefei 230027, PR China \label{USTC} \and
Department of Physics and Astronomy, University of South Carolina, SC 29208, Columbia, USA \label{USC} \and
Universit\'e Grenoble Alpes, CNRS, Grenoble INP, SIMAP, 38402 Saint Martin d'H\'eres, France \label{UGA} 
}
 

